Explainable Verbal Reasoner Plus (EVR+): A Natural Language Reasoning Framework that Supports Diverse Compositional Reasoning

Languages models have been successfully applied to a variety of reasoning tasks in NLP, yet the language models still suffer from compositional generalization. In this paper we present Explainable Verbal Reasoner Plus (EVR+), a reasoning framework that enhances language models' compositional reasoning ability by (1) allowing the model to explicitly generate and execute symbolic operators, and (2) allowing the model to decompose a complex task into several simpler ones in a flexible manner. Compared with its predecessor Explainable Verbal Reasoner (EVR) and other previous approaches adopting similar ideas, our framework supports more diverse types of reasoning such as nested loops and different types of recursion. To evaluate our reasoning framework, we build a synthetic dataset with five tasks that require compositional reasoning. Results show that our reasoning framework can enhance the language model's compositional generalization performance on the five tasks, using a fine-tuned language model. We also discussed the possibility and the challenges to combine our reasoning framework with a few-shot prompted language model.

==> stale/cartesian_product.tex <==
\subsubsection{Cartesian Product}
Figure \ref{fig:walkthrough_cartesian} shows the flow of EVR+ to solve the cartesian product problem. The EVR+'s episodic memory and external memory is initialized with the background of the problem. Then programs are generated and executed. The problem is eventually solved after a few cycles. 

\paragraph{Episodic Memory State 1 $\rightarrow$ 2} The initial episodic buffer specifies the task (``cartesian''), the available information in the external memory (``chunk$\_$0'') and the goal (``List the items that each person had.''). Given the episodic memory state, the program generator generates the program. \textit{$\#$0 = 'Who are the persons?'} is a sub-goal that can be used to solve the original problem. Then \textit{new$\_$mem(episodic$\_$buffer$\_$1, $\#$0);} starts a new recursion process, and the new episodic memory is initialized with the content in \textit{episodic$\_$buffer$\_$1} and the local variable $\#$0.

\paragraph{Episodic Memory State 2 $\rightarrow$ 3} Given the new episodic memory in the recursion, the program generator generates the new program to get the persons from chunk$\_$0 and add the persons to the episodic buffer. Note that a \textit{qa} module is called to generate the answer. The input to the \textit{qa} module is the content of chunk$\_$0 (\textit{Each of Matthew Rodriguez and Jonathan Diaz had 8 bananas and 15 puppies.}) and episodic$\_$buffer$\_$1 (\textit{Who are the persons?}). The result of the \textit{qa} module is appended to the episodic buffer, becoming the \textit{episodic$\_$buffer$\_$2} in state 3.

\paragraph{Episodic Memory State 3 $\rightarrow$ 4} 
Since the question \textit{Who are the persons?} in episodic$\_$buffer$\_$1 is solved by the statement \textit{The persons are ['Matthew Rodriguez', 'Jonathan Diaz'].} in episodic$\_$buffer$\_$2, the program generator generates \textit{return(episodic$\_$buffer$\_$2)} to end the current recursion process. 

\paragraph{Episodic Memory State 4 $\rightarrow$ 10} Note that the 
\textit{episodic$\_$buffer$\_$3} of state 4 is returned from state 3. A few states from state 4 to state 10 are not shown here to reduce the size of the figure.
\paragraph{Episodic Memory State 10 $\rightarrow$ 11} Episodic state 10 has 6 episodic pieces. Note that \textit{episodic$\_$buffer$\_$3} and \textit{episodic$\_$buffer$\_$5} are repetitive. We use the command \textit{clear$\_$mem()} to reduce the size of the memory and prevent the size of the memory to grow limitlessly. The result is that \textit{episodic$\_$buffer$\_$3} is removed.

\paragraph{Episodic Memory State 11 $\rightarrow$ Result} 
To get the answer from state 11, EVR+ needs to loop over the names (stored in local variable $\#$0) and the items (stored in local variable $\#$1), and rewrite them to natural language statements. Therefore the program generator generates a nested loop script to finish this. 

==> stale/name.tex <==
Significant progress has been made in Natural Language Understanding (NLU) using deep neural networks. Particularly, the large neural network-based Language Models (LM) has achieved near human performance in several NLU tasks. Moving beyond that, efforts have been made to teach neural networks reasoning. Such reasoning tasks usually require much more than recognizing the shallow patterns in language, but also require the understanding of certain reasoning skills, such as arithmetic reasoning or logic reasoning, and world knowledge, such as commonsense reasoning. 


Despite the promising results achieved by NNs on several reasoning tasks, current NNs still struggle with compositional reasoning tasks, where the original reasoning problem can be solved by firstly decomposing it to several simpler ones then solving each simple problem. In particular, NNs tend to suffer from the compositional generalization issue: when the models are trained on the problems requiring less reasoning steps and tested on the problems requiring more steps, the performance drops drastically. 

In this work, we design experiments to try to answer the following questions in compositional reasoning: (1) how much training data is needed for NNs to learn robust representations in a compositional reasoning tasks with/without intermediate annotations; (2) how hard it is to transfer the knowledge of NNs learned in easier reasoning tasks to harder reasoning tasks; (3) what benefits can be obtained from a carefully designed neuro-symbolic system in compositional reasoning tasks. To answer these questions, we synthesize a diagnostic dataset composed of 6 tasks, each of which has designed OOD examples, and conduct a systematic investigation over a wide variety of models. 

In summary, our contributions are: \\
(1) we design a set of diagnostic synthetic tasks to evaluate the models' performance on compositional reasoning; \\
(2) we show that intermediate annotations are crucial for the models to learn robust representations in compositional reasoning; \\
(3) we show that traditional transfer learning and multi-task learning are inefficient in transferring the knowledge from the previously learned tasks; \\
(4) we present a neuro-symbolic approach that achieved more robust compositional generalization and transfer learning. We hope our investigation could enlighten other researchers to design more robust reasoning frameworks. 
